On the representation of de Bruijn graphs

The de Bruijn graph plays an important role in bioinformatics, especially in the context of de novo assembly. However, the representation of the de Bruijn graph in memory is a computational bottleneck for many assemblers. Recent papers proposed a navigational data structure approach in order to improve memory usage. We prove several theoretical space lower bounds to show the limitation of these types of approaches. We further design and implement a general data structure (DBGFM) and demonstrate its use on a human whole-genome dataset, achieving space usage of 1.5 GB and a 46% improvement over previous approaches. As part of DBGFM, we develop the notion of frequency-based minimizers and show how it can be used to enumerate all maximal simple paths of the de Bruijn graph using only 43 MB of memory. Finally, we demonstrate that our approach can be integrated into an existing assembler by modifying the ABySS software to use DBGFM.

==> tables.tex <==

\begin{algorithm}[p!]
\begin{algorithmic}[1]
\STATE \textbf{Input:} Set of k-mers $S$, minimizer size $\ell<k$
\STATE \textbf{Output:} Sequences of all simple paths in the de Bruijn graph of $S$
 \STATE Perform a linear scan of $S$ to get the frequency of all $l$-mers (in memory)\label{algstep:lmercounting}
 \STATE Define the ordering of the minimizers, given by their frequency in $S$\label{algstep:minimizersorder}
 \STATE Partition $S$ into files $F_m$ based on the minimizer $m$ of each $k$-mer\label{algstep:partition}
 \FOR{each file $F_m$ in increasing order of $m$\;\label{algstep:for-each-file}}
  \STATE $C_m \leftarrow$ $m$-compaction of $F_m$ (performed in memory)\;\label{algstep:compact-graph}
  \FOR{each string $u$ of $C_m$}
    \STATE $B_{min} \leftarrow $ min(\lmin($u$),\rmin($u$))\;\label{algstep:bmin}
    \STATE $B_{max} \leftarrow $ max(\lmin($u$),\rmin($u$))\;
    \IF{$B_{min} \le m \text{ and } B_{max} \le m$}
        \STATE Output $u$\;\label{algstep:output}
    \ELSIF{$B_{min} \le m \text{ and } B_{max} > m$}
        \STATE Write $u$ to $F_{B_{max}}$\;
    \ELSIF{$B_{min} > m \text{ and } B_{max} > m$}
        \STATE Write $u$ to $F_{B_{min}}$\;\label{algstep:movemin}
    \ENDIF
   \ENDFOR
   \STATE Delete $F_m$
  \ENDFOR
  \end{algorithmic}
  \caption{\bcalm: Enumeration of all maximal simple paths in the \dbg\label{alg:bcalm}}
\end{algorithm}

\newpage


\begin{table}[p!]
\begin{minipage}{\linewidth}
\setlength{\tabcolsep}{12pt}
\centering
\small
\begin{tabulary}{\linewidth}{@{}LLLL@{}}
\toprule
Dataset & \DSK &
\bcalm & 
\dbgfm 
 \\
\midrule
\multirow{2}{*}{Chromosome 14} & 
%memory & 
43 MB & % dsk mem
19 MB & % bcalm mem
38 MB % dbgfm mem
 \\
 & 
 %time  & 
25 mins & % dsk time
15 mins &% bcalm time
7 mins  \\

\multirow{2}{*}{Whole human genome}& 
%memory  &
1.1 GB & % dsk mem
43 MB &  % bcalm mem
1.5 GB   % bwtdisk mem is 1 G, DBGFM mem is 1.4 GB
\\
 & 
 %time &
5 h & %dsk time % note: 1 thread, my desktop, /scratch, lost the logfile so I just know it's ~310min, arguments: "-t 2 -m 1000 -d 300000 -optimism 1"
12 h & %bcalm time
7 h  \tabularnewline % bwtdisk time, my desktop, hard drive (did another run with USB-SSD and 1.5 GB, 7 hours too)

\bottomrule \\
\end{tabulary}
\end{minipage}
\caption{
Running times (wall-clock) and memory usage of \DSK, \bcalm and \dbgfm  construction on the human chromosome 14 and whole human genome datasets ($k=55$ and $\ell=10$ for both).
\label{tbl:pipelineanalysis}}
% human BWTdisk 1G, k=26 bcalm output: real    1588m20.576s user    1176m11.878s sys     557m18.866s
% DSK: here are k=55 full human running time/mem with SSD: 84 mins, 1.1 GB, 2456744129 solid kmers
% BWTdisk with -m 10000 for human_untrimmed-k55-solid3.linearSeqs: 319m
% DBGFM of human_untrimmed-k55-solid3.linearSeqs:1403.84 MB :\ 8mins computation of dbgfm
% human_untrimmed-k55-solid3.linearSeq: 88240850 simple paths
% BWTDisk -m 1500 full human k=55 m3 my desktop SSD: 403m37.254s
% Bcalm k=55 m3 full human my desktop HDD: 708m52.480s ; 43 MB ; 40309282 simple paths
% just for info: BWTDisk human k=55 minia-output default parameters (256 MB) on cyberstar: 3084m
% chr14 k=55: 639808 simple paths
% human *reference* (concatenated_chrs) k=55: 12914807 simple paths (agrees with minia-graph: 12916747)
\end{table}

\newpage

\begin{table}[p]
\begin{minipage}{\linewidth}
\setlength{\tabcolsep}{12pt}
\centering
\small
\begin{tabulary}{\linewidth}{@{}LLLL@{}}
\toprule
 & DBGFM & Salikhov~\emph{et al.} 
 %& \hspace{10pt} Bowe~\emph{et al.}$^*$ \hspace{10pt} 
 &  Conway \& Bromage \\
\midrule
chr14 & 
38.0 MB  &  % dbgfm 
94.9 MB &   % salikhov
$>875$ MB \\

Full human dataset &  
1462 MB  &  % bcalm mem from table above
2702 MB  & % salikhov
$>22951$ MB    % conway bromage
\\
\bottomrule \\
\end{tabulary}
\end{minipage}
\caption{
Memory usage of de Bruijn graph data structures, on the human chromosome 14 and whole human genome datasets ($k=55$ for both).
We did not run the algorithm of Conway and Bromage because our machine does not have sufficient memory
for the whole genome.
Instead, we report the theoretical size of their data structure, assuming that it would be constructed from the output of \DSK.
As described in~\cite{conway_succinct_2011},
this gives a lower bound on how well their implementation could perform.
\label{tbl:externalcomparison}}
%For the DBGFM and Salikhov~\emph{et al.}, the actual memory usage of the respective implementations is reported. 
%$^*$ Theoretical memory usage is reported: 
%$4m$ bits for Bowe~\emph{et al.}~\cite{sadakane} and 
%the lower bound of $n\lg({4^k \choose n})$ bits for Conway and Bromage~\cite{conway_succinct_2011}, where %$m$ and 
% $n$ %are
%is the number of 
%$(k+1)$-mers and 
%$k$-mers.
% for salikhov: I'm using 8.6 bits per 27-mer and 8.8 bits per 55-mer
% for conway bromage: http://www.wolframalpha.com/input/?i=log2%28+%284%5E55+choose+2456744129%29+%29%2F8%2F1024%2F1024%2F1024
% human k=26: 2572812024 kmers
% human k=55 -t 3: 2456744129 kmers
% chr14 k=55 -t 5: 86319384 kmers

\end{table}


\newpage 

\begin{table}[p]
\begin{minipage}{\linewidth}
\setlength{\tabcolsep}{12pt}
\centering
\small
\begin{tabulary}{\linewidth}{@{}LLLL@{}}
\toprule
 Ordering type  
 & Lexicographical
 & Uniformly Random 
 &   $l$-mer frequency  \\
\midrule 
%Memory usage  & \preliminaryresult{no previous result} MB  &   2.6 GB  & 43 MB   % whole genome
Memory usage  & 804 MB  &  222 MB  & 19 MB   % chr14
\\
%Wall-clock time  & 22m  & 24m  & [not measured, was 29m, but actually was on HDD]   % chr14 ssd running times
%Wall-clock time  & 20m  & 21m  & 15m   % chr14 ssd running times
%\\
\bottomrule \\
\end{tabulary}
\end{minipage}
\caption{
Memory usage %and wall-clock running time 
of \bcalm with three different minimizer orderings: lexicographical, uniformly random, 
and according to increasing \lmer frequencies.
%The dataset used is the whole human genome with $k=55$ and $l=10$.
The dataset used is the human chromosome 14 with $k=55$ and $l=8$.
\label{tbl:ordering}}
%time memused ./hash/bcalm /scratch/bcalm/recomb-datasets/human-k55-m3.dot hash.fullhuman.dot ;  maximal memory used ( kilobyte(s) (K / Kb)) 2641572 ; real    1153m20.185s  user    862m13.332s sys     84m49.305s
\end{table}

\newpage 

\begin{table}[p]
\begin{minipage}{\linewidth}
\setlength{\tabcolsep}{12pt}
\centering
\small
\begin{tabulary}{\linewidth}{@{}LLLLLLLL@{}}
\toprule
 Minimizer size $l$  
 & \ 2
 & 4
 &   6 
 & 8
 &  10 
\\
\midrule
Memory usage  &
9879 MB &   %2 
3413 MB  &   %4
248 MB  &   %6
19 MB  &  %8
19 MB    %10
\\
\revision{Running time} & 
\revision{27m19s} &  % out of mem on rayan-1 & % 2
\revision{22m2s} & %\revision{16m5s} (on rayan-1)& % 4
\revision{20m5s} & %\revision{13m55s} (on rayan-1) & % 6
\revision{18m39s} & %\revision{12m7s}(on rayan-1) & % 8
\revision{21m4s} %\revision{13m53s} (on rayan-1)% 10
% on cyberstar231: 62 mins for m=2, 53 mins for m=4; ~40 mins for m=10
\\
\bottomrule \\
\end{tabulary}
\end{minipage}
\caption{
Memory usage \revision{and wall-clock running time} of \bcalm with increasing values of minimizer sizes $l$ on the chr14 data.
By grouping files into virtual files, these values of $l$ require respectively 4, 16, 64, 256 and 1024 physical files on disk. The ordering of minimizers used is the one based on $l$-mer counts.
\label{tbl:mdependence}}
\end{table}

\newpage 

\begin{table}[p]
\begin{minipage}{\linewidth}
\setlength{\tymax}{0.5\linewidth}
\centering
\small
\begin{tabulary}{\textwidth}{@{}LLLLLLL@{}}
\toprule
Data structure & Memory usage & Bytes\slash \kmer & dBG (B\slash \kmer) & Data (B\slash \kmer) & Overhead (B\slash \kmer) & Run time\\
\midrule
%sparsehash & 2314 MiB & 27.00 & 16   & 8 & 3.00 & 10m49s \\ Shaun's machine
sparsehash & 2429 MB & 29.50 & 16   & 8 & 5.50 & %16m47s \\ % Ec2 m2.4xlarge
\revision{14m4s} \\ % cyberstar21
%DBGFM      & 740 MB  & didn't recompute  & didn't recompute & 8 & didn't recompute & 26m29s \\ % Cyberstar result
\dbgfm      & 739 MB  & 8.98  & 0.53 & 8 & 0.44 & %29m56s \\ % EC2 m2.4xlarge
\revision{21m1s} \\ % cyberstar21
% sparsehash ec2 m2.4xlarge: 435m46s, 73 GB memory, 16.7 million contigs % by the way, memused could not capture mem usage, used `top -d 2 -b | grep -i abyss`
\bottomrule \\
\end{tabulary}
\end{minipage}
\caption{Memory usage and run time (wall clock) of the ABySS hash table implementation (sparsehash) and of the \dbgfm implementation, 
%maxk = 64
using a single thread to process the human chromosome 14 data
set. 
The dBG bytes/$k$-mer column corresponds to the space taken by encoded $k$-mers for  sparsehash, and the FM-index for \dbgfm. The Data bytes/$k$-mer column corresponds to associated data. The Overhead bytes/$k$-mer corresponds to the hash table and heap overheads, as well as the rank/select bit array.
The run time of the \dbgfm row does not
include the time to construct the \dbgfm representation.}
\label{tbl:abyssdbgfm}
%abyss-dbgfm chr14: dbgfm has (43.642322 MB) 26m29.927s memory: 740232 KB
% on ec2, for some reason, the sparsehash full human run gave me these results: maximal memory used ( kilobyte(s) (K / Kb)) 9999316 real    425m44.669s
\end{table}


